Physics Informed Capsule Enhanced Variational AutoEncoder for Underwater Image Enhancement

We present a novel dual-stream architecture that achieves state-of-the-art underwater image enhancement by explicitly integrating the Jaffe-McGlamery physical model with capsule clustering-based feature representation learning. Our method simultaneously estimates transmission maps and spatially-varying background light through a dedicated physics estimator while extracting entity-level features via capsule clustering in a parallel stream. This physics-guided approach enables parameter-free enhancement that respects underwater formation constraints while preserving semantic structures and fine-grained details. Our approach also features a novel optimization objective ensuring both physical adherence and perceptual quality across multiple spatial frequencies. To validate our approach, we conducted extensive experiments across six challenging benchmarks. Results demonstrate consistent improvements of $+0.5$dB PSNR over the best existing methods while requiring only one-third of their computational complexity (FLOPs), or alternatively, more than $+1$dB PSNR improvement when compared to methods with similar computational budgets. Code and data \textit{will} be available at https://github.com/iN1k1/.

==> tables/lsui_l400.tex <==
\begin{table*}[t]
        \centering
        \caption{Quantitative comparison of \myalgoname and state-of-the-art methods on the full-reference lsui dataset ($\uparrow$ higher is better, $\downarrow$ lower is better). For each metric/dataset the best method is in red, the second best in blue.}
        \label{tab:lsui_metrics}
        \footnotesize
\begin{tabularx}{\linewidth}{lCCHHHHHC}
\toprule
                    & PSNR $\uparrow$            & SSIM $\uparrow$           & UIQM $\uparrow$           & UCIQE $\uparrow$          & LPIPS $\downarrow$        & NIQE $\downarrow$          & BRISQUE $\downarrow$       & CLIP-IQA $\uparrow$       \\
\midrule
 RGHS               & 18.65 ± 2.79            & 0.82 ± 0.10            & 2.59 ± 0.50            & \tblfirst{0.62 ± 0.04}  & 0.27 ± 0.09            & 5.74 ± 1.71             & 26.08 ± 9.84            & 0.65 ± 0.23            \\
 UDCP               & 13.35 ± 3.83            & 0.58 ± 0.17            & 2.03 ± 0.55            & 0.59 ± 0.05            & 0.36 ± 0.11            & 6.07 ± 1.88             & 28.61 ± 9.96            & 0.61 ± 0.23            \\
 UIBLA              & 18.03 ± 4.68            & 0.74 ± 0.18            & 2.31 ± 0.71            & 0.60 ± 0.05            & 0.32 ± 0.13            & 6.34 ± 3.21             & 28.22 ± 11.74           & 0.65 ± 0.22            \\
 UGAN               & 19.78 ± 4.01            & 0.80 ± 0.11            & 3.01 ± 0.43            & 0.59 ± 0.06            & 0.34 ± 0.13            & 6.82 ± 1.72             & 30.74 ± 8.25            & 0.62 ± 0.22            \\
 Cluie-Net          & 18.88 ± 2.66            & 0.80 ± 0.08            & 2.99 ± 0.34            & 0.60 ± 0.05            & 0.30 ± 0.10            & 5.14 ± 1.22             & 25.02 ± 8.76            & 0.66 ± 0.23            \\
 TWIN               & 20.11 ± 2.83            & 0.81 ± 0.09            & \tblsecond{3.04 ± 0.35} & 0.61 ± 0.04            & 0.31 ± 0.07            & \tblsecond{4.49 ± 0.97}  & \tblfirst{19.79 ± 7.74}  & 0.64 ± 0.24            \\
 UShape-Transformer & 23.64 ± 3.50            & 0.84 ± 0.10            & 2.96 ± 0.40            & 0.59 ± 0.04            & 0.27 ± 0.07            & 4.93 ± 1.24             & \tblsecond{21.99 ± 7.96} & 0.63 ± 0.23            \\
 Spectroformer      & 20.41 ± 3.92            & 0.81 ± 0.11            & 3.04 ± 0.30            & \tblsecond{0.61 ± 0.04} & 0.30 ± 0.10            & 5.03 ± 1.16             & 24.40 ± 8.34            & 0.69 ± 0.21            \\
 CE-VAE             & 25.32 ± 3.65            & 0.86 ± 0.08            & 2.98 ± 0.42            & 0.59 ± 0.04            & 0.23 ± 0.07            & 5.32 ± 1.30             & 26.10 ± 7.09            & 0.66 ± 0.23            \\
 DM-Underwater      & \tblsecond{27.74 ± 4.40} & 0.90 ± 0.08  & \tblfirst{3.06 ± 0.42}  & 0.59 ± 0.04            & \tblsecond{0.18 ± 0.10} & 5.14 ± 1.49             & 23.80 ± 8.72            & 0.64 ± 0.25            \\
 WF-Diff            & 24.98 ± 5.00            & 0.88 ± 0.10            & 3.00 ± 0.43            & 0.58 ± 0.04            & 0.22 ± 0.12            & \tblfirst{21.87 ± 85.31} & 35.71 ± 34.35           & 0.51 ± 0.26            \\
 PA-Diff            & 26.30 ± 4.30            & \tblsecond{0.90 ± 0.07} & 2.98 ± 0.46            & 0.59 ± 0.04            & \tblfirst{0.16 ± 0.08}  & 5.31 ± 1.62             & 23.16 ± 8.83            & \tblsecond{0.71 ± 0.26} \\
 pi-CE-VAE          & \tblfirst{27.81 ± 3.44}  & \tblfirst{0.91 ± 0.06}            & 2.92 ± 0.46            & 0.59 ± 0.04            & 0.20 ± 0.06            & 5.65 ± 2.10             & 24.86 ± 10.79           & \tblfirst{0.72 ± 0.23}  \\
\bottomrule
\end{tabularx}
\end{table*}

==> tables/performance_vs_latent_space.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabularx}{\linewidth}{l C C C C}
    \toprule
    Method & PSNR $\uparrow$ & On-device Storage [MB] $\downarrow$ & Maximum Recording Duration [h] $\uparrow$ &Transmission time [s] $\downarrow$ \\
    \midrule
    Cluie-Net~\cite{li2023cluienet} & 18.71  & 1.57 & 0.39  & 0.01256 \\
    TWIN~\cite{liu2022twin} & 19.84 & 1.57  & 0.39 &  0.01256 \\
    UShape-T.~\cite{peng2023ushape-lsuidataset} & \tblsecond{23.02}  & \tblsecond{1.57} & \tblsecond{0.39} & \tblsecond{0.01256} \\
    Spectr.~\cite{khan2024spectroformer} & 20.09 &1.57 & 0.39 & 0.01256  \\
    CEVAE & \tblfirst{24.49} & \tblfirst{0.52} &  \tblfirst{1.17} &   \tblfirst{0.00416} \\
    \myalgoname & &  1.04 &  & 0.00832 \\
    \bottomrule
\end{tabularx}
\caption{Enhancement performance and storage/transmission capabilities. Considering the real-world LSUI-L400 dataset, for a $256 \times 256$ input image, we computed the corresponding device storage space required for enhanced image generation and the related transmission time on a 1 GBbps bandwidth beacon. We also report on the maximum recording duration that would fit an off-the-shelf commercial device \protect\footnotemark ($\uparrow$ higher is better, $\downarrow$ lower is better).
}
\label{tab:psnr_vs_compression}
\end{table}
